Multi-dimensional fractional wave equation and some properties of its fundamental solution

In this paper, a multi-dimensional fractional wave equation that describes propagation of the damped waves is introduced and analyzed. In contrast to the fractional diffusion-wave equation, the fractional wave equation contains fractional derivatives of the same order $\alpha,\ 1\le \alpha \le 2$ both in space and in time. This feature is a decisive factor for inheriting some crucial characteristics of the wave equation like e.g. a constant phase velocity of the damped waves that are described by the fractional wave equation. Some new integral representations of the fundamental solution of the multi-dimensional wave equation are presented. In the one- and three-dimensional cases, the fundamental solution is obtained in explicit form in terms of elementary functions. In the one-dimensional case, the fundamental solution is shown to be a spatial probability density function evolving in time. However, for the dimensions grater than one, the fundamental solution can be negative and therefore does not allow a probabilistic interpretation anymore. To illustrate analytical findings, results of numerical calculations and numerous plots are presented.

==> def.tex <==
\newcommand{\FTS}[2]{\frac{{\textstyle #1}}{{\textstyle #2}}}
\newcommand{\nat}{I\!\!N}
\newcommand{\NN}{I\!\!N}
\newcommand{\ka}{I\!\!K}
\newcommand{\rgr}{{\rm grad}}
\newcommand{\ce}{I\!\!\!\!C}
\newcommand{\CC}{I\!\!\!\!C}
\newcommand{\re}{I\!\!R}
\newcommand{\RR}{I\!\!R}
 \newcommand{\intl}{\int\limits}
\newcommand{\suml}{\sum\limits}
\setcounter{page}{1}
\thispagestyle{empty}
%%%%  DEFINITIONS by F. MAINARDI  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \font\title=cmbx10 scaled \magstep2
\font\bfs=cmbx10 scaled \magstep2
\def\eg{{\it e.g.}\ } \def\ie{{\it i.e.}\ }
\def\sg{\hbox{sign}\,}
\def\sgn{\hbox{sign}\,}
\def\sign{\hbox{sign}\,}
\def\e{\hbox{e}}
\def\exp{\hbox{exp}}
\def\ds{\displaystyle}
\def\dis{\displaystyle}
\def\q{\quad}	 \def\qq{\qquad}
\def\lan{\langle}\def\ran{\rangle}
\def\l{\left} \def\r{\right}
\def\lra{\Longleftrightarrow}
\def\arg{\hbox{\rm arg}}
\def\d{\partial}
 \def\dr{\partial r}  \def\dt{\partial t}
\def\dx{\partial x}   \def\dy{\partial y}  \def\dz{\partial z}
%% \def\lim{\hbox{lim}}
\def\rec#1{{1\over{#1}}}
\def\log{\hbox{\rm log}\,}
\def\erf{\hbox{\rm erf}\,}     \def\erfc{\hbox{\rm erfc}\,}
%%%% DEFINITION for the GREEN FUNCTION G_{\alpha,\beta}^\theta}
%%%% and their Fourier/Laplace transforms
\def\G{{G_{\alpha,\beta}^\theta}}
\def\K{K_{\alpha,\beta}^\theta}
\def\Gxt{\G (x,t)}
\def\Gkt{{\widehat{\G}}  (\kappa,t)}
\def\Gxs{{\widetilde{\G}}  (x,s)}
\def\Gks{{\widehat{\widetilde {\G}}} (\kappa,s)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\FT{{\cal F}\,} %% FOURIER TRANSF
\def\LT{{\cal L}\,}  %% LAPLACE TRANSF
\def\L{{\cal L}} %%% Laplace Transform !!!!
\def\F{{\cal F}} %%% Fourier Transform !!!!
\def\M{{\cal M}}  %%% Mellin Transform
\def\I{{\cal I}}  %% The generic open interval	\in \RR
%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pni{\par \noindent}
\def\vsh{\smallskip}
\def\vs{\medskip}
\def\vvs{\bigskip}
\def\vvvs{\bigskip\medskip} %% {\vskip 1.5truecm}
\def\vsp{\par}
\def\vsn{\vsh\pni}
\def\cen{\centerline}
\def\ra{\item{a)\ }} \def\rb{\item{b)\ }}   \def\rc{\item{c)\ }}
%%%%%%%%%%%%%%%%%%%
%%% DEF of BINOMIAL COEFFICIENTS
\def\alphak{{\alpha \choose k}}
\def\alphazero{{\alpha \choose 0}}
\def\alphaone{{\alpha \choose 1}}
\def\alphatwo{{\alpha \choose 2}}
\def\alphakk{{\alpha \choose k+1}}
